An asynchronous parallel high-throughput model calibration framework for crystal plasticity finite element constitutive models

Crystal plasticity finite element model (CPFEM) is a powerful numerical simulation in the integrated computational materials engineering (ICME) toolboxes that relates microstructures to homogenized materials properties and establishes the structure-property linkages in computational materials science. However, to establish the predictive capability, one needs to calibrate the underlying constitutive model, verify the solution and validate the model prediction against experimental data. Bayesian optimization (BO) has stood out as a gradient-free efficient global optimization algorithm that is capable of calibrating constitutive models for CPFEM. In this paper, we apply a recently developed asynchronous parallel constrained BO algorithm to calibrate phenomenological constitutive models for stainless steel 304L, Tantalum, and Cantor high-entropy alloy.

==> fig/uq_workflow.tex <==

\begin{center}
\smartdiagramset{
set color list={orange!60, blue!50!cyan,magenta!60,green!50!lime!60},
circular distance=5cm,
font=\large,
text width=6.5cm,
% module minimum width=2.5cm,
module minimum height=1.5cm,
% arrow line width=5pt,
arrow tip=to,
}
\centering
\smartdiagram[circular diagram]{
% \smartdiagramadd[circular diagram:counterclockwise]{
  \textbf{\texttt{MultilevelEstimators.jl}}  \\
  \begin{itemize}
  \small
    \vspace{-0.2cm} \item multi-level/-index Monte Carlo
    \vspace{-0.2cm} \item adaptive unbiased estimator
    \vspace{-0.2cm} \item uncertainty quantification
  \normalsize
  \end{itemize}
  ,
  \textbf{\texttt{DREAM.3D}}  \\
  \begin{itemize}
  \small
  	\vspace{-0.2cm} \item sample microstructure RVE
    \vspace{-0.2cm} \item crystallography texture
    \vspace{-0.2cm} \item mesh resolution
  \normalsize
  \end{itemize}
  ,
  \textbf{\texttt{DAMASK}}  \\
  \begin{itemize}
  \small
    \vspace{-0.2cm} \item materials constitutive models
    \vspace{-0.2cm} \item crystal plasticity finite element
    \vspace{-0.2cm} \item PETSc numerical solvers
  \normalsize
  \end{itemize}
}
% {
% above right of module1/return QoI(s), 
% below left of module2/query input,
% % above of module3/QoI(s),
% }

% \smartdiagramconnect{->}{module1/module2}
% \smartdiagramconnect{-to,bend right,shorten >=8pt,shorten <=8pt,"no"{midway,above right,text=black}}{module1/module2} 
% \smartdiagramconnect{->}{module2/module1}
% \smartdiagramconnect{->}{module3/module1}

% \smartdiagramadd[circular diagram:clockwise]{B,C,A}{
% right of module1/Text 1 without arrow, 
% above of module1/Text 2,
% left of module3/Text 3,
% above left of module3/Text 4,
% below left of module2/{Something}}
\end{center}


